The Greatest Teacher, Failure is: Using Reinforcement Learning for SFC Placement Based on Availability and Energy Consumption

Software defined networking (SDN) and network functions virtualisation (NFV) are making networks programmable and consequently much more flexible and agile. To meet service level agreements, achieve greater utilisation of legacy networks, faster service deployment, and reduce expenditure, telecommunications operators are deploying increasingly complex service function chains (SFCs). Notwithstanding the benefits of SFCs, increasing heterogeneity and dynamism from the cloud to the edge introduces significant SFC placement challenges, not least adding or removing network functions while maintaining availability, quality of service, and minimising cost. In this paper, an availability- and energy-aware solution based on reinforcement learning (RL) is proposed for dynamic SFC placement. Two policy-aware RL algorithms, Advantage Actor-Critic (A2C) and Proximal Policy Optimisation (PPO2), are compared using simulations of a ground truth network topology based on the Rede Nacional de Ensino e Pesquisa (RNP) Network, Brazil's National Teaching and Research Network backbone. The simulation results showed that PPO2 generally outperformed A2C and a greedy approach both in terms of acceptance rate and energy consumption. A2C outperformed PPO2 only in the scenario where network servers had a greater number of computing resources.

==> sections/results-old.tex <==
In this section, we present the results of the SFC placement using two RL algorithms, A2C and PPO. Firstly, we describe the simulation scenario and the parameters used in the experiments. Then, we present the results of the algorithms parametrization. Finally, we present the results of algorithms for different scenario configurations.

\subsection{Simulation Setup}
\label{subsec:simulation-setup}

To perform the experiments in this paper, we build a simulator using the Python language in other to generate the SFC requests, server failures, and repair events. The arrival of SFC requests follows a Poisson process with a constant arrival rate $\lambda$. The lifetime of SFC requests follows an exponential function with rate $1/\mu$, where $\mu$ is the average lifetime \cite{li2018context}. To represent a diverse range of customers, each customer has their own arrival rate and average SFC lifetime. 

The failure and repair events of the servers and VFNs follow an exponential function with failure rate and arrival rate, respectively \cite{torquato2019iaas,lima2020data}. However, others PDFs can be used, if required. The failure rate is defined by $1/MTTF$, where $MTTF$ corresponds to either to the servers or the VNFs. The repair rate is defined by $1/MTTR$, where the servers and the VNFs each have their respective values. Table \ref{tab:simulation-parameters} summarizes the parameters used in the simulations. It is important to highlight that our simulator allows these parameters be easily changed to represent different scenarios.


\begin{table}[ht]
\caption{Simulation Parameters}
\centering
\label{tab:simulation-parameters}
\begin{tabular}{@{}cc@{}}
\toprule
\textbf{Parameter}                  & \textbf{Value} \\ \midrule
Number of servers                   &50               \\
Number of resources per server      &10                \\
Server MTTF                         &8760h                \\
Server MTTF                         &1.667h                \\
VNF MTTF                            &2880h                \\
VNF MTTR                            &0.17h                \\
Energy consumption (CPU)            &40W                \\
Energy consumption (memory)         &30.17W                \\
Maximum number of redundant VNFs     &4                \\
Number of customers                 &5                \\
Arrival rate ($\lambda$)            & 0.04 request/h                \\
SFC lifetime ($\mu$)                 &1000h  \\
\bottomrule
\end{tabular}
\end{table}


We consider a network with 50 physical servers, each with 10 computational resources available to deploy VFNs from SFC requests. We consider server MTTF and MTTR of 8760 hours and a 1.667 hours, respectively. For the VNFs, we consider parameters of generic virtual machines, with MTTF equal to 2880 hours and MTTR equal to 0.17 hours. The MTTF and MTTR parameters were gathered from \cite{araujo2014availability}. For the energy consumption, we consider CPU and memory consumption of 40W and 30.17W, respectively \cite{ali2015energy}. The energy consumption increases linearly as new VNFs are added in the SFC placement. The maximum number of redundant VNFs of the same type equals four.

The arrival rate $\lambda$ is four SFC requests per 100 hours, while the SFC lifetime is 1000 hours \cite{palhares2014joint}.
In a simulation, an SFC is generated randomly for each customer composed of two or three VNFs from the types previously defined; $\lambda$ and $\mu$ parameters are generated based on the standard values described previously. To generate these parameters, we consider a uniform distribution with lower and upper bounds equal to plus and minus 10\% of the standard value of $\lambda$ and $\mu$.

We consider a fixed number of customers equal to five. We consider three different VNF types: a Wide Area Network-optimizer (WAN-opt), a firewall, and an Intrusion Detection System (IDS), as shown in Table \ref{tab:vnf-types}. The firewall and IDS requires one computational resource from the server, while WAN-opt requires four computational resources from the servers \cite{xu2018energy}. 

\begin{table}[h]
\centering
\caption{VNF types}
\label{tab:vnf-types}
\begin{tabular}{@{}cc@{}}
\toprule
VFN type                              & Resources required to deploy \\ \midrule
Intrusion Detection System (IDS)      & 1                            \\
Firewall                              & 1                            \\
Wide Area Network-optimizer (WAN-opt) & 4                            \\ \bottomrule
\end{tabular}
\end{table}

In this study, we compare two different RL algorithms: A2C and PPO. In the following subsections we will describe the results of parametrization experiments and the application of these algorithms in different scenarios.


\subsection{Parametrization Results}
First, the algorithms were configured with their respective parameters. We varied two common parameters of both algorithms that impact their learning process: the learning rate ($\alpha$) and the discount factor ($\gamma$). 

The algorithms are implemented using the Stable Baselines library\footnote{\url{https://stable-baselines.readthedocs.io/en/master/index.html}}. Stable Baselines is a Python library that provides a set of improved implementations of RL algorithms based on OpenAI Baselines. The source code used to perform the experiments of this study is available at GitHub\footnote{\url{https://github.com/GutoL/SFC_RL}}. The other parameters are provided by the library based (from the original publications of algorithms). The variation of $\alpha$ and $\gamma$ are based on the standard values, and are shown in Table \ref{tab:alpha-gamma-variation}. The PPO used in this study is the second version named PPO2 provided by Stable Baselines framework \footnote{\url{https://stable-baselines.readthedocs.io/en/master/modules/ppo2.html}}.

\begin{table}[h]
\caption{$\alpha$ and $\gamma$ variation for parametrization}
\label{tab:alpha-gamma-variation}
\centering
\begin{tabular}{@{}cc@{}}
\toprule
Parameter & Variation                             \\ \midrule
$\alpha$  & 0.00005, 0.00025, 0.0005, 0.00075 \\
$\lambda$ & 0.85, 0.9, 0.99, 0.95            \\ \bottomrule
\end{tabular}
\end{table}

% https://artint.info/2e/html/ArtInt2e.Ch12.S6.html
We consider the SFC placement as an episodic task for training the algorithm, where one episode is approximately one year of customer requests. We carried out 30 experiments to train the agent. For the algorithm training, we consider 8760 steps (the number of hours in one year) multiplied by 10. To evaluate the training convergence of algorithms, we consider the cumulative reward, the sum of all rewards received so far, as a function of the number of steps. Figure \ref{fig:parametrization-ppo2} and \ref{fig:parametrization-a2c} show the parametrization results for the cumulative reward metric for A2C and PPO2, respectively.

\begin{figure*}[h]
\centering
    \begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{figures/results/parametrization/A2C/g=0.9_a=5e-05.png}
    \caption{}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{figures/results/parametrization/A2C/g=0.9_a=0.00025.png}
    \caption{}
    \end{subfigure}
    
    %
    \begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{figures/results/parametrization/A2C/g=0.9_a=0.0005.png}
    \caption{}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{figures/results/parametrization/A2C/g=0.9_a=0.00075.png}
    \caption{}
    \end{subfigure}
\caption{Parameter variation of A2C algorithm}
\label{fig:parametrization-a2c}
\end{figure*}


%------------------------------------------------------------------------------


\begin{figure*}
\centering
    \begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{figures/results/parametrization/PPO2/g=0.9_a=5e-05.png}
    \caption{}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{figures/results/parametrization/PPO2/g=0.9_a=0.00025.png}
    \caption{}
    \end{subfigure}
    
    %
    \begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{figures/results/parametrization/PPO2/g=0.9_a=0.0005.png}
    \caption{}
    \end{subfigure}
    %
    \begin{subfigure}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{figures/results/parametrization/PPO2/g=0.9_a=0.00075.png}
    \caption{}
    \end{subfigure}
\caption{Parameter variation of PPO2 algorithm}
\label{fig:parametrization-ppo2}
\end{figure*}

For all combinations of parameters, both algorithms converge as we have a fast cumulative reward growth following some steps. For the A2C algorithm, the $\alpha$ value that obtained the best results was 0.00025 (Figure \ref{fig:parametrization-a2c}b), while the highest $\alpha$ value tested resulted in the worst accumulated reward results (Figure \ref{fig:parametrization-a2c}d). The discount factor $\gamma$ did not present significant impact in the cumulative reward for the A2C algorithm. All the values evaluated had very similar behavior, but $\gamma=0.99$ resulted in better cumulative rewards.

Similar to the A2C algorithm, the $\alpha$ value of 0.00025 for the PPO2 obtained the highest cumulative rewards. As shown in Figure \ref{fig:parametrization-ppo2}, the discount factor $\gamma$ for the PPO2 has a greater impact than in A2C. For instance, with $\alpha=0.00005$ (Figure \ref{fig:parametrization-a2c}a), the cumulative reward for $\gamma=0.85$ grows faster than all other $\gamma$ values.
In contrast to the A2C algorithm, $\gamma=0.85$ resulted in the greatest cumulative reward for the PPO2 algorithm.

For both algorithms, the most appropriate learning rate was 0.00025. Finding an appropriate learning rate value is an important step in adjusting the RL algorithms. As per Equation \ref{eq:q-update}, the learning rate $\alpha$ controls the adjustment made to the parameters of the policy function. Thus, very small values can cause a vanish gradient, while very large values can cause an exploding gradient. Both compromise the RL agent's learning. Indeed, for both algorithms, $\alpha=0.00075$ and $\alpha=0.00005$ resulted in a slow cumulative reward growth, but $\alpha=0.00025$ resulted in fast cumulative reward growth.

Comparing the discount factor $\gamma$, the PPO2 algorithm presented best results with a small $\gamma$, while the A2C algorithm presented the best results with higher values of $\gamma$. The discount factor determines the importance of future rewards for the current state at a given stage, which can influence the agent learning, as described in the Subsection \ref{subsec:reinforcement-learning-bkg}. Therefore, for the SFC placement problem, the A2C algorithm worked better giving less importance to future rewards, while the PPO2 algorithm worked better giving more importance to future rewards.

When one compares the convergence velocity of both algorithms i.e. the speed at which the accumulated reward grows, the PPO2 algorithm outperformed the A2C algorithm. Figure \ref{fig:parametrization-a2c}b and Figure \ref{fig:parametrization-ppo2}b show that the cumulative reward of the PPO2 algorithm starts to grow with fewer steps than the A2C algorithm. While both algorithms achieve the cumulative reward of 100000, the PPO2 algorithm achieves this faster. After defining more suitable parameters for both algorithms, we can compare them in different SFC placement problem scenarios.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Scenario Variation Results}
In this section, we evaluate the performance of A2C and PPO2 algorithms in two different network topologies, each with different parameters. We vary the number of resources of servers and the number of customers sending SFC requests to the service provider.

The main goal is to evaluate two metrics: the \textbf{acceptance rate} and the \textbf{energy consumption} of system. The acceptance rate metric is the number of SFC requests allocated in the system that met the customer availability requirements. The energy consumption metric is the sum of energy consumption for all SFC requests allocated in the system. These metrics are considered in the reward function \ref{eq:reward}. 

We carried out 30 simulations for training the agent and evaluate it. Again, the number of steps used to train the RL agent is 8760 (the number of hours in one year) multiplied by 10. After training, we reset the environment by removing all VNFs allocated during the training and create new customers randomly as outlined in Subsection \ref{subsec:simulation-setup}. We then test the agent for a period of one year.

\subsubsection{Random network topology}
Firstly, we assess the RL algorithms in a network with 50 servers as per \cite{palhares2014joint}. We use the same configuration as per Table \ref{tab:simulation-parameters} but vary the number of available resources in servers and the number of customers sending SFC requests.

Figure \ref{fig:50-nodes-resource-units-variation} shows the results when the number of available resources increases. As the number of resources per server increases, the acceptance rate increases too, as shown in \ref{fig:50-acceptation-rate-resources}. As more resources are available, the RL agent can allocate more redundant VNFs thus increasing availability, and as a result meeting the customer's SLA requirements. 

%--------------------------------------------------
\begin{figure}[h]
  \centering
  \subfloat[Acceptance rate]{\includegraphics[width=0.5\textwidth]{figures/results/scenario_variation/50_nodes/resources_Acceptance Rate.png}\label{fig:50-acceptation-rate-resources}}
  \hfill
  \subfloat[Energy consumption]{\includegraphics[width=0.5\textwidth]{figures/results/scenario_variation/50_nodes/resources_Energy Consumption (W).png}\label{fig:50-energy-consumption-resources}}
  \caption{Resource units variation for the network with 50 nodes}
  \label{fig:50-nodes-resource-units-variation}
\end{figure}

When there are five resources per server, the median acceptance rate is 85.44\% for PPO2 and 90.12\% for A2C. However, when the number of resources increases to 10, the median acceptance rate increases to  97.50\% for PPO2 and to 97.38\% for A2C. At 15 resources per server, the median acceptance rate increases to 97.78\% and 97.80\% for PPO2 and A2C. Clearly, increasing the number of resources available per server results in gains up to a certain limit. When we increase the number of resources per server from five to 10 , we have a maximum increase of 12\%, for PPO2, in the acceptance rate. However, when we increase the number of available resources from 10 to 15, the increase is approximately 1\%. From that point on, an investment in the acquisition of servers with more available resources will result in a marginal increases in the acceptance rate, and may not result in cost savings for the service provider.

From a performance perspective, both techniques achieved very similar result with the exception of the scenario with five resources per server. In this scenario, the A2C outperformed the PPO2 in terms of median acceptance rate. However, as the number of available resources increases, the median acceptance rate become very close, and statistically similar.

Figure \ref{fig:50-energy-consumption-resources} shows the total energy consumption for all SFCs allocated for each algorithm. Similar to the acceptance rate, the energy consumption increases as the number of available resources increases. More redundant VNFs are allocated when the number of available resources in the servers increases. As a result, the energy consumption increases. For example, when the number of available resources increases from five to 10, the median energy consumption increases from 7227.51W to 8104.64W for the PPO2, and from 7192.43W to 8244.98W for the A2C. However, as the number of available resources increases from 10 to 15, energy consumption remains the same for both algorithms. The increase in energy consumption can translate into OPEX increases for service providers. However, we can also see an increase of approximately 5\% in the acceptance rate when we increase the number of resources from 5 to 10, as well as an increase in energy consumption around 1000W. Thus, the SFC service provider needs to assess whether this increase in the acceptance rate justifies the increase in energy consumption and the acquisition of more computational resources e.g. more servers or higher quality servers. Similarly, the service provider may consider increasing the price charged to the customer for higher availability. 

Figure \ref{fig:50-nodes-customers-variation} shows the results when the number of customers sending SFC requests increases. As can be seen in Figure \ref{fig:50_acceptation-rate-customers}, the acceptance rate decreases considerably from c.97\% for four customers to c.76\% for 32 customers. As the number of SFC requests increases, the available server resources are consumed faster. The reduction of available resources makes it more difficult for the RL agent to allocate the SFC and consequently meeting customer availability requirements. 

%--------------------------------------------------
\begin{figure}[h]
  \centering
  \subfloat[Acceptance rate]{\includegraphics[width=0.5\textwidth]{figures/results/scenario_variation/50_nodes/customers_Acceptance Rate.png}\label{fig:50_acceptation-rate-customers}}
  \hfill
  \subfloat[Average Energy consumption]{\includegraphics[width=0.5\textwidth]{figures/results/scenario_variation/50_nodes/customers_Energy Consumption (W).png}\label{fig:50_energy-consumption-customers}}
  \caption{Number of customers variation for the network with 50 nodes}
  \label{fig:50-nodes-customers-variation}
\end{figure}
%--------------------------------------------------

In general, comparing PPO2 and A2C performance by median acceptance rate, we can see that for a small number of customers (four and six) the A2C outperformed the PPO2. However, as the number of customers increase, the PPO2 outperforms the A2C.

As shown in Figure \ref{fig:50_energy-consumption-customers}, the increase in customer numbers increased the energy consumption by allocated SFCs considerably. This is not suprising. As more SFC requests arrive in the system, more SFCs are allocated thereby increasing energy consumption. For instance, consider four customers in the system, the median energy consumption is 6876.66W for the PPO2 and 6631.07W for A2C. When the number of customers increases to 32, the median energy consumption increases to 42593.19W for the PPO2 and 40031.99W for A2C. It is worth noting that the energy consumption and acceptance rate behave very similarly i.e. the lower the acceptance rate, the lower the energy consumption. As such, in terms of energy consumption, the A2C algorithm performed better than PPO2.

\subsubsection{Real network topology}
In order to evaluate the RL algorithms performance in a real network topology, we consider the Hibernia Atlantic Network in Northern Ireland. The topology of the Hibernia Atlantic Network is composed of 17 nodes (Figure \ref{fig:ireland-network}). It was extracted from topology zoo\footnote{http://www.topology-zoo.org/dataset.html}. We used the same methodology to train the RL algorithms used in the previous scenarios.

\begin{figure}[ht]
\centering
\includegraphics[width=0.5\columnwidth]{figures/HiberniaNireland.jpg}
\caption{Hibernia Atlantic Network topology}
\label{fig:ireland-network}
\end{figure}

Figure \ref{fig:17-acceptation-rate-resources} shows the acceptance rate as the number of available resources in servers increases. The median acceptance rate for five resources was 74.46\% for the PPO2 and 76.00\% for the A2C. The A2C algorithm outperformed the PPO2 when there are five resources per server for SFC placement. However, when the number of available resources increases to 10, the median acceptance rate increased to about 96.08\% for the PPO2 and 96.23\% for the A2C, an increase of 21.62\% and 20.23\%, respectively. In constrast to the topology with 50 nodes, the A2C outperformed the PPO2 when we consider a server with only 10 resources to deploy SFCs. 

%--------------------------------------------------
\begin{figure}[h]
  \centering
  \subfloat[Acceptance rate]{\includegraphics[width=0.4\textwidth]{figures/results/scenario_variation/17_nodes/resources_Acceptance Rate.png}\label{fig:17-acceptation-rate-resources}}
  \hfill
  \subfloat[Average Energy consumption]{\includegraphics[width=0.4\textwidth]{figures/results/scenario_variation/17_nodes/resources_Energy Consumption (W).png}\label{fig:17-energy-consumption-resources}}
  \caption{Resource units variation}
  \label{fig:17-nodes-resources-variation}
\end{figure}

Where the server had 15 resources, the median acceptance rate was 97.83\% for PPO2 and 97.78\% for A2C, representing a small increase of 1.75\% and 1.55\%, respectively, when compared to the scenario with 10 available resources. In addition, at 15 available resources per server, although the both algorithms achieve very similar results, the PPO2 outperformed the A2C in terms of median acceptance rate.

When we examine the energy consumption of deployed SFCs (Figure \ref{fig:17-energy-consumption-resources}), at five resources per server, the energy consumption is c.6000W; the energy consumption of A2C is slightly higher than PPO2. The energy consumption increases to  c.8000W with 10 available resources per server and stabilises after this point. This stabilisation of energy consumption is expected since the acceptance rate does not increase considerably when we increase the number of server resources from 10 to 15.

%It is important highlight that when we reduce the number of servers in the network, i.e., to decrease the number of available resources to allocate the SFCs, the acceptance rate is impacted. For instance, comparing Figures \ref{fig:50-acceptation-rate-resources} and \ref{fig:17-acceptation-rate-resources}, when we have five resources per servers, the median of acceptance rate for the network with 50 nodes is around 85-90\%, while it is around 75\% for the network with 17 servers, the maximum difference of 10\%. On the other hand, this difference in the acceptance rate is reflected in the energy consumption of the SFCs allocated. Considering the servers with five resources, the energy consumption is around 7000W (Figure \ref{fig:50-energy-consumption-resources}) for the network with 50 servers and 6000W for the network with 17 servers (Figure \ref{fig:17-energy-consumption-resources}), a difference of 1000W.

Figure \ref{fig:17-acceptation-rate-customers} shows the acceptance rate as the number of customers in the system increases based on the Hibernia Atlantic Network topology. The acceptance rate is experiences a significant impact, decreasing from approximately 97\% to c.69\%, a reduction of 27\%. In addition, we can see that the performance of the algorithms is statistically very similar. Considering a scenario with four customers, PPO2 achieved a worse median acceptance rate than A2C at 95.60\% and 97.06\%, respectively. In contrast, at 32 customers (worst case evaluated), PPO2 obtained a better median acceptance rate compared to A2C at 69.89\% and 67.07\%, respectively. For 16 and 32 customers, one can see a greater difference in the performance of the algorithms in terms of median acceptance rate, with the PPO2 outperforming the A2C algorithm.

%--------------------------------------------------
\begin{figure}[h]
  \centering
  \subfloat[Acceptance rate]{\includegraphics[width=0.4\textwidth]{figures/results/scenario_variation/17_nodes/customers_Acceptance Rate.png}\label{fig:17-acceptation-rate-customers}}
  \hfill
  \subfloat[Average Energy consumption]{\includegraphics[width=0.4\textwidth]{figures/results/scenario_variation/17_nodes/customers_Energy Consumption (W).png}\label{fig:17-energy-consumption-customers}}
  \caption{Number of customers variation}
  \label{fig:17-nodes-customers-variation}
\end{figure}

%--------------------------------------------------

Figure \ref{fig:17-energy-consumption-customers} shows the energy consumption variation as the number of customers sending SFC requests increases. The energy consumption increases from  c.6000W for four customers to  c.37000W for 32 customers. In addition, we can see that the increase in energy consumption follows the behavior of the acceptance rate. For instance, with 32 customers, where the PPO2 achieved a higher acceptance rate than the A2C, the median energy consumption of PPO2 is 37435.70W, while the median energy consumption of A2C algorithm is 35155.17W, a difference of 2280.53W.

In general, the performance of A2C and PPO2 are statistically similar based on the acceptance rate and energy consumption in the scenarios evaluated. However, when one considers the median acceptance rate, the A2C outperformed the PPO2 when we vary the the number of resources per server in the infrastructure. When we varied the number of customers sending requests, the PPO2 achieved better acceptance rate levels than A2C. Therefore, in the scenarios with a high number of customers sending requests, the PPO2 algorithm is the more suitable technique due to its higher  acceptance rate.
